Seeing Hate Differently: Hate Subspace Modeling for Culture-Aware Hate Speech Detection

Hate speech detection has been extensively studied, yet existing methods often overlook a real-world complexity: training labels are biased, and interpretations of what is considered hate vary across individuals with different cultural backgrounds. We first analyze these challenges, including data sparsity, cultural entanglement, and ambiguous labeling. To address them, we propose a culture-aware framework that constructs individuals' hate subspaces. To alleviate data sparsity, we model combinations of cultural attributes. For cultural entanglement and ambiguous labels, we use label propagation to capture distinctive features of each combination. Finally, individual hate subspaces, which in turn can further enhance classification performance. Experiments show our method outperforms state-of-the-art by 1.05\% on average across all metrics.

==> RelatedWork.tex <==
\section{Related Work}
\textbf{Hate Speech Detection.} 
ss
\\

\noindent \textbf{Cultural Considerations in Hate Speech Detection.} 
CREHate~\cite{lee2023exploring} collected posts and hired various annotator from four geographical diverse English-speaking countries to label them. From the pairwise label agreement ratios in Figure~\ref{fig:agreement}, we can observe that annotators from different countries have different perception of hate. ~\cite{lee2023hate}

